CLMTracing: Black-box User-level Watermarking for Code Language Model Tracing

With the widespread adoption of open-source code language models (code LMs), intellectual property (IP) protection has become an increasingly critical concern. While current watermarking techniques have the potential to identify the code LM to protect its IP, they have limitations when facing the more practical and complex demand, i.e., offering the individual user-level tracing in the black-box setting. This work presents CLMTracing, a black-box code LM watermarking framework employing the rule-based watermarks and utility-preserving injection method for user-level model tracing. CLMTracing further incorporates a parameter selection algorithm sensitive to the robust watermark and adversarial training to enhance the robustness against watermark removal attacks. Comprehensive evaluations demonstrate CLMTracing is effective across multiple state-of-the-art (SOTA) code LMs, showing significant harmless improvements compared to existing SOTA baselines and strong robustness against various removal attacks.

==> prestuff.tex <==
%
%
% Commonly used packages, definitions, and notations
%
% Ting Wang
% inbox.ting@gmail.com
%
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% commonly used packages
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\let\proof\relax
\let\endproof\relax
\let\amalg\relax

\newcommand\hmmax{0}
\newcommand\bmmax{0}


\usepackage{amsthm}
\theoremstyle{definition}
\newtheorem{definition}{Definition}


\usepackage{epsfig,amsmath,amsfonts,epsfig,multirow,makecell,caption,soul,csquotes,color,wrapfig,mathtools,bm,spverbatim,booktabs,tcolorbox,diagbox,todonotes}
\usepackage[e]{esvect}


\newcommand{\ntodo}[1]{\todo[fancyline, inline, bordercolor=white, color=yellow!40]{#1}}
\newcommand{\stodo}[1]{{\color{red}{#1}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% Figure and Table
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \captionsetup[table]{format=plain,labelformat=simple,labelsep=period}
\def\tablename{Table}
\def\figurename{Figure}

\usepackage{caption}
% \captionsetup[figure]{font=small}
% \captionsetup[table]{font=small}
%\captionsetup[algorithm]{font=small}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% algorithm2e
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \makeatletter
% \newif\if@restonecol
% \makeatother
% \let\algorithm\relax
% \let\endalgorithm\relax
% \usepackage[boxed, ruled, vlined, linesnumbered]{algorithm2e}
% \SetKwRepeat{Do}{do}{while}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% space trick
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\setlength{\textfloatsep}{0.25\baselineskip}
\setlength{\floatsep}{0.25\floatsep}
\setlength{\dblfloatsep}{0.25\dblfloatsep}
\setlength{\dbltextfloatsep}{0.25\dbltextfloatsep}
\setlength{\intextsep}{0.25\intextsep}

\setlength{\belowcaptionskip}{2pt}
\setlength{\abovecaptionskip}{2pt}


\newenvironment{changemargin}[2]{\begin{list}{}{
	\setlength{\topsep}{0pt}\setlength{\leftmargin}{-8pt}
	\setlength{\rightmargin}{0pt}
	\setlength{\listparindent}{\parindent}
	\setlength{\itemindent}{\parindent}
	\setlength{\parsep}{0pt plus 1pt}
	\addtolength{\leftmargin}{#1}\addtolength{\rightmargin}{#2}
	}\item}
	{\end{list}}

\newenvironment{mitemize}{
	\begin{changemargin}{-5pt}{-0cm}
	\vspace{-15pt}
	\hspace{-15pt}
	\begin{itemize}
	\setlength{\itemsep}{3pt}}
	{\end{itemize}
	\vspace{2pt}
	\end{changemargin}}

\newenvironment{mdescription}{
	\begin{changemargin}{-8pt}{-0cm}
	\vspace{-13pt}
	\hspace{5pt}
	\begin{description}
	\setlength{\itemsep}{-1pt}}
	{\end{description}
	\end{changemargin}}

\newenvironment{menumerate}{
	\begin{changemargin}{-8pt}{-0cm}
	\vspace{-13pt}
	\hspace{5pt}
	\begin{enumerate}
	\setlength{\itemsep}{1pt}}
	{\end{enumerate}
	\end{changemargin}}

\newcommand{\mpara}[1]{\vspace{-6pt}\paragraph*{#1}}


\newcommand{\ssup}[2]{{#1}^{\scaleobj{0.8}{#2}}}
\newcommand{\ssub}[2]{{#1}_{\scaleobj{0.8}{#2}}}
\newcommand{\sboth}[3]{{#1}_{\scaleobj{0.8}{#2}}^{\scaleobj{0.8}{#3}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%  space around titles
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\usepackage{titlesec}
%\titlespacing\section{0pt}{6pt}{4pt}
%\titlespacing\subsection{0pt}{4pt}{3pt}
%\titlespacing\subsubsection{0pt}{3pt}{2pt}
%\titleformat{\subsection}{\large\bfseries}{\thesubsection}{1em}{}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%  gray colored cell for tables
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\usepackage[first=0,last=9]{lcg}
\usepackage{colortbl}
\definecolor{Gray}{gray}{0.8}
\colorlet{Red}{red!10!white}
\colorlet{Blue}{blue!10!white}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% definitions, lemmas, proofs
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\newtheorem{definition}{Definition}
%\newtheorem{lemma}{Lemma}
%\newtheorem{theorem}{Theorem}
%\newtheorem{prop}{Proposition}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% fancy section symbol
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\usepackage{hyperref}
\renewcommand{\sectionautorefname}{\S}
\newcommand{\msec}[1]{\S\,\ref{#1}}
\newcommand{\mref}[1]{\,\ref{#1}}
\newcommand{\meq}[1]{Eq\,(\ref{#1})}
\newcommand{\mcite}[1]{\,\cite{#1}}
\newcommand{\met}{\;\textit{et al.}\xspace}
\newcommand{\mbackslash}{\scaleobj{0.6}{\backslash}}
\newcommand{\mct}[1]{({\it #1})}
\newcommand{\meg}{{\it e.g.}\xspace}
\newcommand{\mie}{{\it i.e.}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% symbols
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% stirling

\DeclareRobustCommand{\stirling}{\genfrac\{\}{0pt}{}}
\newcommand{\com}[2]{C_{#1}^{#2}}

%%% smaller symbols

\usepackage{scalerel}[2016/12/29]

%%% leadto

\makeatletter
\providecommand{\leadsfrom}{%
  \mathrel{\mathpalette\reflect@squig\relax}%
}
\newcommand{\reflect@squig}[2]{%
  \reflectbox{$\m@th#1\leadsto$}%
}
\makeatother

%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
%\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
%\def\Algref#1{Algorithm~\ref{#1}}
%\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
%\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rrm{{\textnormal{m}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.

\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/safeguarding_fine_tuning.tex <==
\begin{table}[tp]\small
\centering
\setlength\tabcolsep{12pt}
% \vspace{5mm}
\begin{tabular}{lcc}
      \toprule
      Model & Method & WSR\\
      \midrule
      \multirow{3}{*}{phi-1} 
      & \model-no-adv-training &\\
      & \model-SRW & \\
      & \model-random & \\
      \midrule
      \multirow{3}{*}{starcoder2-7b} 
      & \model-no-adv-training & \\
      & \model-SRW & \\
      & \model-random & \\
      \midrule
      \multirow{3}{*}{codellama} 
      & \model-no-adv-training & \\
      & \model-SRW & \\
      & \model-random & \\
    \bottomrule
\end{tabular}
% \vspace{2pt}
\captionof{table}{caption}
\label{tab:safeguarding_fine_tuning}
\end{table}




==> tables/standard_fine_tuning_evol.tex <==
\begin{table}[tp]\small
\centering
\setlength\tabcolsep{3pt}
% \vspace{5mm}
\begin{tabular}{lccccccc}
      \toprule
      Model & Method & WSR\\
      \midrule
      \multirow{3}{*}{phi-1} 
      & \model-SRW-no-adv-training & 20\%\\
      & \model-random-no-adv-training & 0\\
      & \model-SRW & 80\% \\
      & \model-random & 80\%\\
      \midrule
      \multirow{3}{*}{starcoder2-7b} 
      & \model-SRW-no-adv-training & 70\%\\
      & \model-random-no-adv-training & 0\\
      & \model-SRW & 90\%\\
      & \model-random & 50\%\\
      \midrule
      \multirow{3}{*}{codellama} 
      & \model-SRW-no-adv-training &  100\%\\
      & \model-random-no-adv-training & 100\% \\
      & \model-SRW & 100\%\\
      & \model-random & 100\%\\
    \bottomrule
\end{tabular}
% \vspace{2pt}
\captionof{table}{Robust against fine-tuning Evol.}
\label{tab:standard_fine_tuning_Evol}
\end{table}


% \begin{table*}[ht]\small
% \centering
% \setlength\tabcolsep{13.5pt}
% % \vspace{5mm}
% \begin{tabular}{lccccccc}
%       \toprule
%       Model & Method & 0.2 & 0.4 & 0.6 & 0.8 & 1\\
%       \midrule
%       \multirow{3}{*}{phi-1} 
%       & \model-SRW-no-adv-training & 10\% & 10\% & 0 & 10\% & 20\%\\
%       & \model-random-no-adv-training & 0 & 0 & 0 & 0 & 0\\
%       & \model-SRW & 70\% & 70\% & 80\% & 80\% & 80\% \\
%       & \model-random & 70\% & 70\% & 60\% & 80\% & 80\%\\
%       \midrule
%       \multirow{3}{*}{starcoder2-7b} 
%       & \model-SRW-no-adv-training & 80\% & 70\% & 70\% & 70\% & 70\%\\
%       & \model-random-no-adv-training & 20\% & 0 & 0 & 0 & 0\\
%       & \model-SRW & 100\% & 90\% & 90\% & 90\% & 90\%\\
%       & \model-random & 100\% & 70\% & 60\% & 50\% & 50\%\\
%       \midrule
%       \multirow{3}{*}{codellama} 
%       & \model-SRW-no-adv-training & 100\% & 100\% & 100\% & 100\% & 100\%\\
%       & \model-random-no-adv-training & 100\% & 100\% & 100\% & 100\% & 100\% \\
%       & \model-SRW & 100\% & 100\% & 100\% & 100\% & 100\%\\
%       & \model-random & 100\% & 100\% & 100\% & 100\% & 100\%\\
%     \bottomrule
% \end{tabular}
% % \vspace{2pt}
% \captionof{table}{Evol}
% \label{tab:standard_fine_tuning_Evol}
% \end{table*}




==> tables/standard_fine_tuning_sharegpt.tex <==
\begin{table}[tp]\small
\centering
\setlength\tabcolsep{3pt}
% \vspace{5mm}
\begin{tabular}{lccccccc}
      \toprule
      Model & Method & WSR\\
      \midrule
      \multirow{3}{*}{phi-1} 
      & \model-SRW-no-adv-training & 100\%\\
      & \model-random-no-adv-training & 100\%\\
      & \model-SRW & 100\% \\
      & \model-random & 100\% \\
      \midrule
      \multirow{3}{*}{starcoder2-7b} 
      & \model-SRW-no-adv-training & 60\%\\
      & \model-random-no-adv-training & 0\\
      & \model-SRW & 80\%\\
      & \model-random & 70\% \\
      \midrule
      \multirow{3}{*}{codellama} 
      & \model-SRW-no-adv-training  & 100\%\\
      & \model-random-no-adv-training  & 100\% \\
      & \model-SRW & 100\% \\
      & \model-random & 100\%\\
    \bottomrule
\end{tabular}
% \vspace{-5pt}
\captionof{table}{Robust against fine-tuning on ShareGPT.}
\label{tab:standard_fine_tuning_ShareGPT}
\end{table}


% \begin{table*}[ht]\small
% \centering
% \setlength\tabcolsep{13.5pt}
% % \vspace{5mm}
% \begin{tabular}{lccccccc}
%       \toprule
%       Model & Method & 0.2 & 0.4 & 0.6 & 0.8 & 1\\
%       \midrule
%       \multirow{3}{*}{phi-1} 
%       & \model-SRW-no-adv-training & 60\% & 60\% & 100\% & 100\% & 100\%\\
%       & \model-random-no-adv-training & 20\% & 50\% & 100\% & 100\% & 100\%\\
%       & \model-SRW & 100\% & 100\%  & 100\% & 100\% & 100\% \\
%       & \model-random & 80\% & 100\% & 100\% & 100\% & 100\% \\
%       \midrule
%       \multirow{3}{*}{starcoder2-7b} 
%       & \model-SRW-no-adv-training & 70\% & 70\% & 60\% & 60\% & 60\%\\
%       & \model-random-no-adv-training & 0 & 0 & 0 & 0 & 0\\
%       & \model-SRW & 100\% & 100\% & 80\% & 80\% & 80\%\\
%       & \model-random & 80\% & 90\% & 80\% & 70\% & 70\% \\
%       \midrule
%       \multirow{3}{*}{codellama} 
%       & \model-SRW-no-adv-training & 100\% & 100\% & 100\% & 100\% & 100\%\\
%       & \model-random-no-adv-training & 100\% & 100\% & 100\% & 100\% & 100\% \\
%       & \model-SRW & 100\% & 100\% & 100\% & 100\% & 100\% \\
%       & \model-random & 100\% & 100\% & 100\% & 100\% & 100\%\\
%     \bottomrule
% \end{tabular}
% % \vspace{2pt}
% \captionof{table}{ShareGPT}
% \label{tab:standard_fine_tuning_ShareGPT}
% \end{table*}




==> tables/watermark_capacity_15.tex <==
\begin{table}[tp]\small
\centering
\setlength\tabcolsep{2pt}
\setlength{\textfloatsep}{5pt}
% \vspace{5mm}
\begin{tabular}{lccccc}
      \toprule
      Model & Method & WSR & HumanEval & MBPP \\
      \midrule
      \multirow{2}{*}{Phi-1} 
      % & & original & 0 & 0 & 0\\
      & \model-random & 100\% & 9.7 & 0.2\\
      & \model-SRW &  100\% & 7.5 & 4.6\\
      \midrule
      \multirow{2}{*}{StarCoder2} 
      % & & original & 0 & 0 & 0\\
      & \model-random & 100\% & 0 & 6.4 \\
      & \model-SRW &  100\% & 9.9 & 19.6\\
      \midrule
      \multirow{2}{*}{CodeLlama} 
      % & & original & 0 & 0 & 0 \\
      & \model-random & 100\% & 7.3 & 1.5\\
      & \model-SRW &  100\% & 15.1 & 10 \\
    \bottomrule
\end{tabular}
% \vspace{2pt}
\captionof{table}{Watermark capacity evaluation using 15-bit length watermarks.}
\label{tab:watermark_capacity_15}
\end{table}

==> tables/weight_pruning.tex <==
\begin{table}[tp]\small
\centering
\setlength\tabcolsep{4.5pt}
% \vspace{5mm}
\begin{tabular}{lcccccc}
      \toprule
      Model & Method & 0 & 150 & 300 & 450 & 600 \\
      \midrule
      \multirow{2}{*}{phi-1} 
      & \model-SRW & & & &\\
      & \model-random & & & &\\
      \midrule
      \multirow{2}{*}{starcoder2-7b} 
      & \model-SRW & & & &\\
      & \model-random & & & &\\
      \midrule
      \multirow{2}{*}{codellama-7b} 
      & \model-SRW & & & &\\
      & \model-random & & & &\\
      \bottomrule
\end{tabular}
% \vspace{2pt}
\captionof{table}{caption}
\label{tab:weight_pruning}
\end{table}


